Dynamically Relative Position Encoding-Based Transformer for Automatic Code Edit

Adapting Deep Learning (DL) techniques to automate non-trivial coding activities, such as code documentation and defect detection, has been intensively studied recently. Learning to predict code changes is one of the popular and essential investigations. Prior studies have shown that DL techniques such as Neural Machine Translation (NMT) can benefit meaningful code changes, including bug fixing and code refactoring. However, NMT models may encounter bottleneck when modeling long sequences, thus are limited in accurately predicting code changes. In this work, we design a Transformer-based approach, considering that Transformer has proven effective in capturing long-term dependencies. Specifically, we propose a novel model named DTrans. For better incorporating the local structure of code, i.e., statement-level information in this paper, DTrans is designed with dynamically relative position encoding in the multi-head attention of Transformer. Experiments on benchmark datasets demonstrate that DTrans can more accurately generate patches than the state-of-the-art methods, increasing the performance by at least 5.45\%-46.57\% in terms of the exact match metric on different datasets. Moreover, DTrans can locate the lines to change with 1.75\%-24.21\% higher accuracy than the existing methods.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/old_intro.tex <==
\section{intro}

% AI in code
Deep Learning (DL) techniques have been adapted to solve many traditional software engineering problems and tasks recently \cite{ferreira2021software,yang2020survey}, e.g., fault localization\cite{eniser2019deepfault,li2019deepfl,wardat2021deeplocalize}, automatic program repair\cite{lutellier2019encore,li2020dlfix,gupta2017deepfix}, code summarization \cite{ahmad2020transformer,leclair2020improved,wan2018improving}, code prediction \cite{kim2021code, huang2020commtpst}, and defect prediction\cite{hasanpour2020software,chen2020software,wang2018deep}. Among these fields, learning from code for code change prediction draws more and more research investigations\cite{islam2019comprehensive,wen2018well}. Precisely 
editing code can significantly facilitate the software maintenance process for developers \cite{tufano2019learning,chakraborty2020codit}. 



% AI in code changes
Code edit throughout the program development and maintenance relates to various behaviours such as code refactor~\cite{tansey2008annotation,meng2015does,ge2012reconciling} and patch generation\cite{lutellier2020coconut,jiang2021cure}.
% In the process of program development and maintenance, code changes are often involved, including API-related changes\cite{nguyen2010graph,nguyen2016api}, refactoring\cite{tansey2008annotation,meng2015does,ge2012reconciling}, and patch generation\cite{lutellier2020coconut,jiang2021cure}. 
Prior research \cite{tufano2019learning,chakraborty2020codit,tufano2018empirical,chen2019sequencer} discovers that code changes generally follow repetitive edit patterns and can be employed to automatically generate targeted code based on original code.
% generate program patch by learning from past code changes.
Figure~\ref{fig:example} presents an example for illustrating the code edit task. In the original code, the method \texttt{testEmpty} needs to return the object's ID and name. However, the functions \texttt{id()} and \texttt{name()} do not exist for the object, which leads to a program bug. The code edit task aims at generating a correct patch for fixing the bug, i.e, changing to corresponding correct functions \texttt{getId()} and \texttt{getName()}, respectively. Due to the syntatic structure of code, automatically identifying the lines for editing and producing accurate edits are challenging.
% However, code change is an extremely long and energy-consuming task for program developers\cite{}, so we need a technology that can automatically predict code changes.


 \begin{figure}[htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/code_example.pdf}
    \caption{An example for illustrating the code edit task. The grey blocks highlight the changed parts in the code.}
    \label{fig:example}
\end{figure}




In recent years, deep learning has made great progress and been applied to many code-related tasks \cite{DBLP:journals/corr/abs-2009-08366,DBLP:conf/kbse/TianLKKLKB20}. The large software engineering datasets, such as GitHub which includes over 100 million repositories with over 200 million merged pull requests (PRs) and 2 billion commits\cite{tufano2019learning}, provide us with sufficient source code for training DL models.
% Using DL in automatic code change prediction is to automate non-trivial coding activities\cite{allamanis2018survey}. It can learn from the history of existing projects to generate a patch for bug fixing or code refactoring.
%Traditional automatic program repair (APR) techniques, such as GenProg\cite{le2011genprog}, are generate-and-validate approaches, which rely on domain-specific knowledge and leverage search space to generate patches and validate the correctness of the generated patches with the guidance of test cases\cite{wen2018context}.
%These features make traditional APR techniques time-consuming\cite{le2017jfix}.
% and not accurate enough\cite{}. \textcolor{green}{i don't konw which paper to cite}
%Comparing with traditional APR techniques, DL-based APR can learn from large software engineering datasets, such as GitHub, which includes over 100 million repositories with over 200 million merged pull requests (PRs) and 2 billion commits\cite{tufano2019learning}. 
Prior studies~\cite{chen2019sequencer,tufano2019empirical,tufano2019learning} have shown that DL techniques such as Neural Machine Translation (NMT)~\cite{bahdanau2014neural} can automatically apply developers' pull request code to generate meaningful code changes.
% , which performs effective in automatic program repair task.
% limit and transformer
NMT models treat pull request code as a series of tokens to learn code change patterns for predicting code edits. However, NMT models have proven ineffective in modeling long sequences~\cite{DBLP:conf/ijcnlp/LeMYM17}, thus may be limited in accurately editting code. 
% ignores the syntactic characteristic of code in statement-level, leading to encounter bottleneck when modeling long sequences, .
For example, in software projects, the code dependencies may have a longer range: one may use a variable that has been declared dozens of lines before. Transformer has proven more effective in capturing long-range sequences than other sequence-to-sequence approaches~\cite{DBLP:conf/iclr/RaePJHL20,DBLP:conf/nips/ZaheerGDAAOPRWY20}. Thus, to mitigate the issue of NMT models and better capture the code dependencies, we propose a novel Transformer-based approach~\cite{vaswani2017attention} for the task.

% . Transformer utilize the attention mechanism to encoder and decoder, which is more effective in capturing long-term dependencies than NMT.





% our approach
% Specifically, we propose a novel model named \tool, a Transformer-based approach to learn the code change activities implemented by developers during pull requests.

\tool takes the code before change and code after change as input, and encodes them to sequences of vectors in the multi-head attention layer of Transformer. To better incorporate the code dependencies, we propose a dynamically relative position encoding strategy to integrate the statement-level information during encoding. 
% \yx{Considering that Transformer is ineffective in capturing program syntactic information in statement-level, which limits the performance in higher-quality patch generation.}
% To better capture the local structure information of code, we propose a dynamically relative position encoding strategy in the multi-head attention of Transformer. 
The proposed position encoding enables Transformer to leverage statement-level syntactic information for generating more accurate code edits. 

To evaluate the performance of our proposed \tool model, we choose three pull request repositories utilized by the work~\cite{tufano2019learning} as benchmark datasets, including Android\cite{android}, Google Source\cite{google}, and Ovirt\cite{Ovirt}. 
Besides, we also involve the 2.3 million 121,895 pair-wise code changes from GitHub open-source projects\cite{tufano2019empirical}.
% Moreover, besides the top-1 accuracy, which represents the accuracy of generating code edits, we additional select BLEU-4\cite{papineni2002bleu} and ROUGE-L\cite{lin2004rouge}, two metrics widely-used in evaluating text generation systems, as performance measurements to evaluate our proposed method.
% , which can well simulate the non-trivial coding activities in evaluating generated code. 
During evaluation, we group project datasets to two levels, i.e., small and medium levels, according to the token numbers of original code following prior studies\cite{cho2014learning,tufano2019empirical,chen2019sequencer}.
% We apply \tool on benchmark datasets to evaluate our effectiveness, and
Experiments demonstrate that \tool accurately predicts more code edits in both small-level and medium-level projects, increasing the performance of the state-of-the-art (SOTA) NMT model \cite{tufano2019learning,tufano2019empirical} by at least 21.42\% and 22.45\% in terms of the exact match metric, respectively. Moreover, \tool successfully locates the lines to change with 10.38\% higher accuracy than the SOTA NMT model. \add{[add results of CODIT?]} 
% 43.63\% of the program patches in small-level projects and 36.61\% in medium-level projects, increasing the performance of the state-of-the-art NMT model by 20.16\% and 20.39\%, respectively.

Overall, we make the following contributions:

\begin{itemize}
    \item We propose \tool, a novel Transformer-based approach to predict code changes.

    \item  We propose a dynamically relative position encoding strategy in the multi-head attention of Transformer, which explicitly incorporates the statement-level syntactic information for better capturing the local structure of code.
    
    \item  We evaluate our approach on benchmark datasets, and the results demonstrate the effectiveness of \tool in predicting accurate code changes.
    
\end{itemize}

\textbf{Paper structure.} We introduce the background in Section~\ref{sec:back}. The proposed approach is illustrated in Section~\ref{sec:method}. Experimental setup and results are depicted in Section~\ref{sec:setup} and Section~\ref{sec:results}, respectively. We show some cases in Section~\ref{sec:case}. The threats to validity and related work are introduced in Section~\ref{sec:threat} and Section~\ref{sec:literature}, respectively. We conclude our work in Section~\ref{sec:con}.
